Policy Finetuning: Bridging Sample-Efficient Offline and Online Reinforcement Learning

Recent theoretical work studies sample-efficient reinforcement learning (RL) extensively in two settings: learning interactively in the environment (online RL), or learning from an offline dataset (offline RL). However, existing algorithms and theories for learning near-optimal policies in these two settings are rather different and disconnected. Towards bridging this gap, this paper initiates the theoretical study of policy finetuning, that is, online RL where the learner has additional access to a "reference policy" $\mu$ close to the optimal policy $\pi_\star$ in a certain sense. We consider the policy finetuning problem in episodic Markov Decision Processes (MDPs) with $S$ states, $A$ actions, and horizon length $H$. We first design a sharp offline reduction algorithm -- which simply executes $\mu$ and runs offline policy optimization on the collected dataset -- that finds an $\varepsilon$ near-optimal policy within $\widetilde{O}(H^3SC^\star/\varepsilon^2)$ episodes, where $C^\star$ is the single-policy concentrability coefficient between $\mu$ and $\pi_\star$. This offline result is the first that matches the sample complexity lower bound in this setting, and resolves a recent open question in offline RL. We then establish an $\Omega(H^3S\min\{C^\star, A\}/\varepsilon^2)$ sample complexity lower bound for any policy finetuning algorithm, including those that can adaptively explore the environment. This implies that -- perhaps surprisingly -- the optimal policy finetuning algorithm is either offline reduction or a purely online RL algorithm that does not use $\mu$. Finally, we design a new hybrid offline/online algorithm for policy finetuning that achieves better sample complexity than both vanilla offline reduction and purely online RL algorithms, in a relaxed setting where $\mu$ only satisfies concentrability partially up to a certain time step.

==> Sections/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{As this is a theoretical paper, we do not foresee any negative societal impacts of our work.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> Sections/plan.tex <==
\section*{Plan}

\begin{enumerate}
  % \item Variance reduction algorithm for $H^3$ setting?
  % \item Algorithm box.
% \item (Done) Proof of main result 1: variance reduction algorithm for $H^3$ setting.
%   \begin{itemize}
%   \item Theorem 1: $H^5SC^\star/\eps^2$ via original VI-LCB.
%   \item Theorem 2: $H^3SC^\star/\eps^2$ via PEVI-ADV.
%   \item High-probability bound for VI-LCB? (For later use). Best if we can adapt directly from~\citep{rashidinejad2021bridging}.
%   \item Make main theorem high-probability too (instead of in expectation)?

%     All the concentration involved: (1) Bernstein concentration, which always holds; (2) concentation of $N_t(s,a)$, may involve some smart Markov inequality (for inverse binomial) with high moments; (3) other concentration.
%   \item Proof about $G(s)$ (main guarantee for the reference value function).
%   \item Bernstein variances are close to true variance of $V_{\rf}$, or upper bounded by $G(s)$. Figure out explicitly what are the necessary concentration events.
%   \item Most other parts similar as Jiantao's proof.
%  \end{itemize}
% \item Shorten algorithm box.
\item Extend $\pi_\star$ to $\mu_+$. Check whether $H^3$ result is correct (or otherwise only $H^5$ result is correct).~\yub{just say this is possible in comments? seems not hard, and not really related to our main point now.}
% \item (Done) Statement + proof of online finetuning lower bound (main result 2).
% \item (Done) Statement + proof of online finetuning $H^3SC^{\rm partial}/\eps^2 + (H-h_\star+1)^3SAC^{\rm partial}/\eps^2$ upper bound (main result 3).
% \item Online upper bound beyond concentrability: $\mu$ satisfies $C^{\rm partial}$ concentrability on all but one $h$. ($C^\star=\infty$ in this case.)
\item Writing:
  \begin{itemize}
  % \item Title. 1: Let offline RL community notice (and cite). 2: Highlight "policy finetuning" concept.
  \item (Tengyang) Prelim, related work, section 3.
  \item (Yu) Section 4, Intro, Section 5.
  \item Conclusions, Abstract, final edits. Paper checklist.
  \end{itemize}
  % Use "Policy finetuning" as storyline, and make offline data collection a special case of policy finetuning.
% How to differentiate with the batch of recent works on \{pessimism, sharp offline learning\}?
% \begin{itemize}
%     \item Our online lower bound is new.
% \end{itemize}
\end{enumerate}
